XAIQA: Explainer-Based Data Augmentation for Extractive Question Answering

Extractive question answering (QA) systems can enable physicians and researchers to query medical records, a foundational capability for designing clinical studies and understanding patient medical history. However, building these systems typically requires expert-annotated QA pairs. Large language models (LLMs), which can perform extractive QA, depend on high quality data in their prompts, specialized for the application domain. We introduce a novel approach, XAIQA, for generating synthetic QA pairs at scale from data naturally available in electronic health records. Our method uses the idea of a classification model explainer to generate questions and answers about medical concepts corresponding to medical codes. In an expert evaluation with two physicians, our method identifies $2.2\times$ more semantic matches and $3.8\times$ more clinical abbreviations than two popular approaches that use sentence transformers to create QA pairs. In an ML evaluation, adding our QA pairs improves performance of GPT-4 as an extractive QA model, including on difficult questions. In both the expert and ML evaluations, we examine trade-offs between our method and sentence transformers for QA pair generation depending on question difficulty.

==> tables/mimicqa_gpt4_table.tex <==
\begin{table*}[h]
  \centering 
  \caption{mimicQA test set results for GPT-4 with synthetic QA pairs.  XAIQA method with ClinicalBERT (CBERT) used for post-processing denoted as PP.
  Exact match denoted as EM.}
  \begin{tabular}{p{2.6cm}p{3.25cm}p{3.25cm}p{3.25cm}}
    \toprule
    \textbf{Method} &                 \textbf{ROUGE} &                    \textbf{F1} &                    \textbf{EM} \\
\midrule
 Zero-Shot & 0.520 [0.497 - 0.543] & 0.600 [0.579 - 0.621] & 0.300 [0.275 - 0.326] \\
CBERT & 0.550 [0.528 - 0.573] & 0.606 [0.586 - 0.627] & 0.314 [0.289 - 0.340] \\
MPNET & 0.556 [0.532 - 0.580] & 0.613 [0.593 - 0.634] & 0.324 [0.298 - 0.349] \\
XAIQA Raw & 0.555 [0.531 - 0.579] & 0.598 [0.577 - 0.620] & 0.316 [0.290 - 0.342] \\
XAIQA PP & 0.562 [0.538 - 0.586] & 0.613 [0.593 - 0.633] & 0.309 [0.285 - 0.333] \\
\bottomrule
  \end{tabular}
      \label{tab:mimicqa_gpt4_table}
  \end{table*}
    
